Liftability and vanishing theorems for Fano threefolds in positive characteristic II

In our series of papers, we prove that smooth Fano threefolds in positive characteristic lift to the ring of Witt vectors. Moreover, we show that they satisfy Akizuki-Nakano vanishing, $E_1$-degeneration of the Hodge to de Rham spectral sequence, and torsion-freeness of Crystalline cohomologies. In this paper, we establish these results except when $|-K_X|$ is very ample and the Picard group is generated by $\omega_X$. To this end, we show that an arbitrary smooth Fano threefold is quasi-$F$-split when the Picard number or the Fano index is larger than one.

==> section10.tex <==
\section{Toward QFS for $V_1$}

How about using the embedding? 
$X \subset P = \P(1, 1, 1, 2, 3)$. 
We have $-K_P \sim \MO_P(8)$ and $-K_X \sim \MO_X(2)$. 

\begin{lem}
Assume $p \geq 3$. 
Let $X$ be $V_1$. 
Then the following hold. 
\begin{enumerate}
    \item $H^1(X, \Omega^1_X(K_X))=0$. 
    \item $H^2(X, \Omega^1_X(-p^iK_X))=0$ for every $i>0$. 
    \item $X$ is quasi-$F$-split. 
\end{enumerate}
%    A smooth Fano threefold of No.~2-6-a is quasi-F-split. 
\end{lem}
\begin{proof}
By Proposition \ref{prop:criterion for qFs} and Lemma \ref{lem:SRC}, it suffices to show (1) and (2). 
% that
% \begin{enumerate}
%     \item[(1)] $H^1(X, \Omega^1_X(K_X))=0$.
%     \item[(2)] $H^2(X, \Omega^1_X(-p^iK_X))=0$ for every $i >0$.
% \end{enumerate}

\medskip


\noindent\textbf{Step 1: Proof of (1).}\,\,  By the conormal exact sequence, we have the following exact sequence:
\[
0\to \sO_X(K_X-X)\to \Omega^1_P|_X(K_X) \to \Omega^1_X(K_X)\to 0.
\]
Since we have 
\[
H^2(X, K_X-X)=H^2(X, \sO_X(-2-6))=0, 
\] 
%by Lemma \ref{lem:vanishing for (2-6-1)},
it suffices to show $H^1(X, \Omega^1_P|_X(K_X))=0$.

Since $P$ is smooth around $X$, we have the following exact sequence:
\[
0\to \Omega^{1}_{P}(K_{P})\to \Omega^{1}_{P}(K_{P}+X)\to \Omega^{1}_{P}|_X(K_{X})\to 0,  
\]
where $\Omega^1_P(K_P)$ is the tensor product. 
Since $P$ is smooth around $X$, the cokernel (appearing only on $X$) does not change even after taking the double dual, i.e., we get 
\[
0\to \Omega^{[1]}_{P}(K_{P})\to \Omega^{[1]}_{P}(K_{P}+X)\to \Omega^{1}_{P}|_X(K_{X})\to 0. 
\]
More explicitly, this seq is exact around $X$, because of the original seq. 
Outside $X$, this seq is clearly exact. 
By Bott vanishing, we have
\begin{itemize}
    \item $H^1(P, \Omega^{[1]}_{P}(K_{P}+X))=0$%H^1(P, \Omega^{[1]}_{P}(-1,-1))=0$ and 
    \item $H^2(P, \Omega^{[1]}_{P}(K_{P}))=0$%^2(P, \Omega^{[1]}_{P}(-3,-3))=0$.
\end{itemize}
% Consider the double dual hom: 
% \[
% \Omega_P^1 \to \Omega_P^{[1]}. 
% \]
% This is isom outside zero-dim (two pts). 
% For 
% \[
% 0 \to K \to \Omega_P^1 \to I \to 0, \qquad 0 \to I \to \Omega_P^{[1]} \to C \to 0, 
% \]
% $K$ and $C$ have zero-dim supports. 
% Hence 
% \[
% H^i(P, \Omega_P^1) \xrightarrow{\simeq} H^i(P, I) 
% \]
%  %Therefore, (1) holds.
% $H^{\geq 2}(\Omega_P^1) \simeq H^{\geq 2}(\Omega_P^{[1]})$. 
% On thet other hand, if $H^0(\Omega_P^{[1]})=H^1(\Omega_P^{[1]})=0$, 
% then $H^1(\Omega_P^1)$ should be $H^0(C)$. 



\medskip


\textbf{Step 2: Proof of (2).}\,\,  
Fix $i \in \Z_{>0}$. 
By the conormal exact sequence, we have the following exact sequence
\[
0 \to \sO_X(-p^iK_X-X) \to \Omega^1_P|_X(-p^iK_X) \to \Omega^1_X(-p^iK_X) \to 0.
\]
We have 
\[
H^3(X, \sO_X(-p^iK_X-X))=H^3(X, \sO_X(2p^i -6)) =0. 
\]
{\cred If $p^i=2$, this is nonzero. 1-dim}

by Lemma \ref{lem:vanishing for (2-6-1)}.
Thus, it suffices to show $H^2(X, \Omega^1_P|_X(-p^iK_X))=0$.

As before, we have the following exact sequence:
\[
0\to \Omega^{[1]}_{P}(-p^i(K_{P}+X)-X)\to \Omega^{[1]}_{P}(-p^i(K_{P}+X))\to \Omega^{1}_{P}|_X(-p^iK_{X})\to 0.
\]
Then 
\begin{itemize}
    \item $H^2(P, \Omega^{[1]}_{P}(-p^i(K_{P}+X)))=H^2(P, \Omega^{[1]}_{P}(2p^i))=0$ by Bott vanishing and 
    \item $H^3(P, \Omega^{[1]}_{P}(-p^i(K_{P}+X)-X))=H^3(P, \Omega^{[1]}_{P}(2p^i-6))= H^0(P, \Omega_P^2(4-2p^i))=0$ by \cite[Proposition 1.3]{Totaro(Fano)}.
\end{itemize}
Therefore, the assertion holds.  
\end{proof}


Assume $p=2$. (1) is OK, i.e., $H^1(X, \Omega_X^1(K_X))=0$. 
We have 
$H^3(P, \Omega^{[1]}_{P}(-p^i(K_{P}+X)))=H^3(P, \Omega^{[1]}_{P}(2p^i))=0$. 
Hence we obtain $H^2(X, \Omega_X^1(-2K_X)) \neq 0$. 
Thus we can not use our criterion for $V_1$. 
By SD, we get $H^1(X, \Omega_X^2(2K_X)) \neq 0$. 
\[
0 \to Z_1\Omega_X^2 \otimes K_X \to F_*(\Omega_X^2(2K_X)) \to B_1\Omega_X^3 \otimes K_X \to 0. 
\]
We have $H^0(B_1\Omega_X^3 \otimes K_X))=0$. 

Let us show $H^1(B_1\Omega_X^3 \otimes K_X)=0$. 
By 
\[
0 \to B_1\Omega_X^3 \to Z_1 \Omega_X^3 \to \Omega_X^3 \to 0, 
\]
we get 
\[
H^1(B_1\Omega_X^3 \otimes K_X) \simeq H^1(Z_1\Omega_X^3 \otimes K_X) \simeq H^1( (F_*\omega_X) \otimes K_X)=0. 
\]
Then 
\[
H^1(Z_1\Omega_X^2 \otimes K_X) \xrightarrow{\simeq}  H^1(F_*(\Omega_X^2(2K_X)) \simeq k.  
\]


How about $B_1\Omega_X^2 \otimes K_X$? In general, $V_1$ should be $F$-split (probably). 
Then I guess that $H^1(X, B_1\Omega_X^2 \otimes K_X)$ depends on the choice of $X$. 
% We have 
% \[
% 0 \to Z_1\Omega_X^1 \to F_*\Omega_X^1 \to B_1\Omega_X^2 \to 0. 
% \]


%Question: general $V_1$ in $p=2$ is q-F-split? 
%I think that $F$-split example should be easy by Fedder. 


UNDER CONSTRUCTION: 
Non-F-split example?: 
\[
f = y^3 + x_0^6+x_1^6+x_2^6 + x_0^2x_1^2x_2^2+ x_0^3x_1^3 + x_1^3 x_2^3 + x_2^3x_0^3 + z^2 +z(x_0^2x_1 + x_1^2 x_2 + x_2^2x_0). 
\]
This is not F-split by Fedder. 

Let us show that this is sm. 
$\partial_y =0$ implies $y=0$. 
We first treat the $z=0$ locus. 
WMA $x_0 \neq 0$ by symmetry. 
Then $\partial_{x_0}$ gives $x_0^2(x_1^3+x_2^3)=0$, i.e., $x_1^3 = x_2^3$. 
If $x_1=0$, then $x_2=0$, which contradicts $f=0$. 
Hence $x_i \neq 0$ for every $i$. 
Then $x_1^3 =x_2^3 = x_0^3$. 
Then $f=x_0^2x_1^2x_2^2 \neq 0$. 


%Next, we treat the locus $x_0 \neq 0$. 
%By $\partial_z$, we get 

Let us treat the case when $z \neq 0$.
We have $y=0$. 
If $x_0 = x_1 = x_2=0$, then contradiction. 
Hence $x_0 \neq 0$. Then $x_1^3 =x_2^3$. 


The computation method is explained in [Okada, Smooth weighted hypersurfaces that are not stably rational, Section 3.1]. 
Assume that $X$ defined by deg $6$ poly $f= f(x_0, x_1, x_2, y, z)$ does not pass thru $[0:0:0:1:0], [0:0:0:0:1]$. 
Moreover, the singular points satisfy $x_0 = x_1 = x_2 =0$. 
Then a sing pt is contained in $U := D_+(y) \cap D_+(z)$. 
In this case, for $Q := zy^{-1}$
\[
k[x_0/Q, x_1/Q, x_2/Q, y^3/z^2, z^2/y^3] (\simeq k[s_0, s_1, s_2, t, t^{-1}] \simeq \A^3_s \times (\A^1_t \setminus \{0\}). 
\]
For example, if 
\[
f = z^2 +y^3 + g(x_0, x_1, x_2), 
\]
then 
\[
\widetilde{f} :=f/Q^6 = (z^2/Q^6) + (y^3/Q^6) + \frac{g(x_0, x_1, x_2)}{Q^6}
\]
\[
=(y^6/z^4) + (y^9/z^6) +  \frac{g(x_0, x_1, x_2)}{Q^6}
= t^2 +t^3 +g(s_0, s_1, s_2). 
\]
Assume the projective normality. 
Then $\partial_t$ implies $t=0$. 



Consider 
\[
f=z^2 + z(g(x_0, x_1, x_2))^2 + y^3 + h(x_0, x_1, x_2). 
\]
Assume that $h_{x_1}(1, x_1, x_2)= h_{x_2}(1, x_1, x_2) =0$ has finitely many solutions (e.g., $h=0$ defines a smooth curve on $\P^2$). 
Then we can avoid these points by a general conic $g(x_0, x_1, x_2)$. 
Then we may assume $x_0=x_1=x_2=0$. 
By $z^2 +y^3=0$, we may assume that $D_+(y) \cap D_+(z)$. 
Then $\widetilde f = t^2 + t(g(s_0, s_1, s_2))^2 +t^3 + h(s_0, s_1, s_2).$ 
$\partial_t=0$ gives $t = g(s_0, s_1, s_2)$. 
By $\partial_{s_i}$, we get $s_0 = s_1 = s_2 =0$. 
Then $t=0$, absurd. Done. 

We want to apply KTY. 
\begin{itemize}
\item Page 8: $\delta_1(f) = \Delta_1(f)$ is given. 
\item Cor 4.19 gives a criterion. $f \in \m^{[2]}$ and $\Delta_1(f) \in \m^{[4]}$ seems to be enough to conclude non-QFS. 
\end{itemize}
Recall that the Witt computation in char 2 is as follows: 
\[
[x]+[y] = (x+y, xy, ...), \quad [x]+[y]+[z] = (x+y+z, xy+yz+zx, ...)
\]
Given two monomials, it suffices to check $\in \m^{[4]}$. 

\begin{prop}
QFS holds for 2-dim. 
\end{prop}

\begin{proof}
%\end{proof}
First, we note that $R/f$ is not $F$-split.
Using $(z,w)^8 \subseteq \m^{[4]}$ and $\Delta_1(f_i) \in (z,w)^{2i}$, we have
\[
f\Delta_1(f) \equiv f_3x^3y^3 +f_2f_3x^2y^3+f_3f_4xy^3+(f_6+f_2f_4)x^3y^2
\]
mod $\m^{[2]}$.
If $f_3 \neq 0$, then there exists a monomial $\alpha \in k[z,w]$ such that $v_{zw}^*(\alpha f_3) \nsubseteq (z,w)^{[2]}$.
We note that $v_d^*(\alpha f)=0$ and
\[
v_d^*(f\Delta_1(f)) =xyv_{zw}^*(\alpha f_3)+yv_{zw}^*(\alpha f_3 f_4).
\]
Thus we have $v_d^*(\alpha f)=0$ and $\phi(\alpha f) \nsubseteq \m^{[2]}$.
By Theorem (Fedder), $ht(R/f)=2$.
\end{proof}

%Probably, the following is smooth F-split: 
%\[
%(x_0+x_1+x_2) yz + y^3 + x_0x_1x_2z + z^2 + x_
%\]

\[
y^2=x^3+f_2(s,t)x^2+f_4(s,t)x+f_6(s,t)
\]

Consider 
\[
f=z^2 + y^3 + yg_1(x_0, x_1, x_2)^4+ g_6(x_0, x_1, x_2). 
\]
WMA: $x_0 = x_1 = x_2 =0$!? 
Then $y \neq 0$. Hence $z \neq 0$. 
On the remaining locus, we have 
\[
f= t^2 +t^3 + tg_1(s_0, s_1, s_2)^4 + g_6(s_0, s_1, s_2).
\]







Set 
\[
g(x_0, x_1, x_2) = x_0^6+x_1^6+x_2^6 + x_0^2x_1^2x_2^2+ x_0^3x_1^3 + x_1^3 x_2^3 + x_2^3x_0^3
\]
Consider the locus $x_0 \neq 0$. 
Set $h(x_1, x_2) :=g(1, x_1, x_2)$. 
$h_{x_1}= x_1^2(1+x_2^3)=0$ implies $x_1=0$ or $x_2^3 =1$. Similarly, $x_2=0$ or $x_1^3=1$. 
Then $(x_1, x_2)=(0, 0)$ or $(x_1^3, x_2^3) =(1, 1)$. 


% \section{Non-$F$-split example in $p=11$}

% Assume $p=11$. 
% Consider 
% \[
% X := \{ x_0^6 +x_1^6 + x_2^6 + x_3^6 +y^2 =0\}\subset \P(1, 1, 1, 1, 3). 
% \]
% We have 
% \[
% D_+(x_0) = \Spec k[\frac{x_1}{x_0}, \frac{x_2}{x_0}, \frac{x_3}{x_0}, \frac{y}{x_0^3}] \simeq \A^4 \subset \P(1, 1, 1, 1, 3)
% \]
% Then 
% \[
% X \cap D_+(x_0) = \{ 1+X_1^6 +X_2^6 + X_3^6 +Y^2=0\}, 
% \]
% which is smooth. 
% Hence a singular point $[a_0:a_1:a_2:a_3:b]$ satisfies $a_0=0$. 
% By symmetry, $a_0= \cdots = a_3=0$. Hence only $[0:0:0:0:1]$ can be a singular point. 
% But $X$ does not pass through this point. Hence $X$ is sm. 


% % We have 
% % \[
% \Gamma(D_+(y), \MO) = 
% (k[x_0, x_1, x_2, x_3, y]_y )_{0} = k[ \frac{x_0^{i_0} x_1^{i_1}x_2^{i_3} x_3^{i_3}}{y^k}], 
% \]
% \begin{itemize}
% \item $k=1$: $x_0^3, x_0^2x_1, x_0x_1x_2$ (up to symmetry). 
% \item $k=2$: $x_0^6, x_0^5x_1, x_0^4x_1x_2, x_0^4x_1^2, ....$
% \end{itemize}
% For $k=2$, we have $x_0^{i_0} x_1^{i_1}x_2^{i_3} x_3^{i_3}$ with 
% $i_0 + i_1 + i_2 + i_3=6$. 
% Then we can divide this into $3+3$, e.g., 
% $x_0^4x_1x_2 = x_0^3 \times x_0x_1x_2$. 
% Therefore, 

% \[
% \Gamma(D_+(y), \MO)  = k[ \frac{x_i^3}{y}, \frac{x_i^2x_j}{y}, \frac{x_ix_jx_k}{y}]. 
% \]
% For $s_i := \frac{x_i^3}{y}, t_{ij}:= \frac{x_i^2x_j}{y}, 
% u_{ijk} = \frac{x_ix_jx_k}{y}$, 
% we get 
% $t_{12}t_{21} = s_1s_2, u_{123}s_1 = t_{12}t_{13}$. 

% Since only $[0:0:0:0:1]$ can be a singular point, 
% but $X$ does not pass through this point. 
% Therefore, $X$ is smooth. 
% %can we apply localisation? 

\begin{prop}
    Let $X=V_1$ and suppose that $C=S\cap S'$ is smooth for general members $S,S'\in |-(1/2)H|$.
    Then $X$ is SRC.
\end{prop}
\begin{proof}
    The member $S$ is isomorphic to a general fibre of a del Pezzo fibration, and thus $S$ is a canonical del Pezzo surface.
    We first show that $H^0(X, \Omega_X^2)=0$.
    Since $|H|$ does not have the base locus, it suffices to show that $H^0(\Omega_X^2|_S)=0$.
    \[
    0\to \Omega_{S}^{[1]}(-H) \to \Omega^2_X|_{S} \to \Omega_{S}^{[2]}.
    \]
    As in Prop 8.3, we have $H^0(S, \Omega_{S}^{[1]}(-H))=0$ since a general member of $|-K_S|$ is smooth by assumption.
    Thus, $H^0(\Omega_X^2|_S)=0$.


    We next show that $X$ is separably uniruled.
    It suffices to show that a smooth Fano threefold $Y$ of No.~2-1 is separably uniruled.
    Since a general fiber is a canonical del Pezzo surface, 
    
    
    Finally, we conclude by [SEPARABLE RATIONAL CONNECTEDNESS AND WEAK APPROXIMATION IN POSITIVE CHARACTERISTIC, Thm 3].
\end{proof}

==> section9.tex <==
\section{Toward lifting}


% \begin{lem}
% Let $V$ be a smooth projective threefold. 
% Assume that $-K_V$ is semi-ample and big. 
% Let $h : V \to W$ be the contraction induced by $-K_V$. 
% If $V$ lifts to $W(k)$, then so is $W$ and $h$.  
% \end{lem}

% \begin{proof}

% \end{proof}


\subsection{Lifting flops}




\begin{thm}
Let $k$ be an algebraically closed field of characteristic $p>0$. 
Let $\psi :Y \to Z$ be a flopping contraction, 
where $Y$ is a smooth threefold. 
Assume that we have a lift $\wt{\psi}: \wt{Y} \to \wt{Z}$ 
of $\psi : Y \to Z$ to $W(k)$. 
Then also the flop $Y^+ \to Z$ lifts to $W(k)$. 
\end{thm}

\begin{proof}
We here only prove the existence of the flop of 
the lifted flopping contraction $\wt{\psi}: \wt{Y} \to \wt{Z}$ (the remaining part will be settled after the proof). 
We follow the strategy of [Tanaka, 
Elliptic sigularities and threefold flops in positive characteristic, Subsection 6.4]. 
More precisely, we shall lift the construction step by step. 




Fix a point $P \in Y$, around which we shall work. 
After taking the completion, we have a finite extension 
\[
k[[x, y, z]] \hookrightarrow \widehat{\MO}_{Z, P}
\]
whose corresponding field extension is Galois. 


Set $A := \MO_Z(Z)$ (affine) and 
we have a $W(k)$-lift $\wt{A}$, 
i.e., $\wt{A}$ is $W(k)$-flat and $\wt{A}/(p)=A$.
Hence we have an $\wt{A}$-module hom ex seq 
\[
0 \to \wt{A} \xrightarrow{\times p} \wt{A} \to A \to 0. 
\]
We have the maximal ideal $\m \subset A$ (corresponding to $P$). 
Then we have the corresponding maximal ideal $\wt{\m}$ of $\wt{A}$. 
Taking the localisation: 
\[
0 \to \wt{A}_{\wt{\m}} \xrightarrow{\times p} \wt{A}_{\wt{\m}} \to A_{\wt{\m}} =?? A_{\m} \to 0. 
\]

Take the $\wt{\m}$-adic completion. 
For the completion of $\wt{C}$ of $\wt{A}_{\wt{\m}}$ 
and $C$ of $A_{\m}$, we  get 
\[
0 \to \wt{C} \xrightarrow{\times p} \wt{C} 
\to C \to 0.  
\]
Since $W(k) \to \wt{A} \to \wt{B} \to \wt{C}$ are all flat, 
$C = \widehat{\MO}_{Z, P}$ has a lift $\wt{C}$. 

Recall that we have a Galois double cover. 
\[
k[[x, y, z]]\hookrightarrow \widehat{\MO}_{Z, P} =C
\]
Fix lifts $\wt{x}, \wt{y}, \wt{z} \in \wt{C}$ of $x, y, z \in C$.  
Since $\wt{x} \mapsto x \in \m $ ($\m$ denotes the maxi ideal of $C$), we get $\wt{x} \in \pi^{-1}(\m)$ for $\pi : \wt{C} \to C$. Hence $\wt{x}$ is contained in the maximal ideal $\wt{\m}$ of $\wt{C}$. 
Since $\wt{C}$ is $\wt{\m}$-adically complete, we get a $W(k)$-algebra homomorphism: 
\[
W(k)[[\wt{x}, \wt{y}, \wt{z}]] \to \wt{C}, \qquad 
\wt{x} \mapsto \wt{x} \quad etc. 
\]
There exists $c \in C$ such that 
\[
C = k[[x, y, z]] \oplus k[[x, y, z]] c. 
\]
Fix a lift $\wt{c} \in \wt{C}$. 
Consider the natural $W(k)[[\wt{x}, \wt{y}, \wt{z}]]$-module hom: 
\[
\theta: W(k)[[\wt{x}, \wt{y}, \wt{z}]] \oplus 
W(k)[[\wt{x}, \wt{y}, \wt{z}]]\wt{c} \to 
\wt{C}
\]

\begin{claim*}
    $\theta$ is isom. 
\end{claim*}

\begin{proof}
Note that 
$\theta$ will become an isom after taking mod $p$, 
and hence $\Im(\theta) + p\wt{C} = \wt{C}$. 
By Nakayama's lemma, $\theta$ is surjective. 
Let us show the injectivity. 
Assume that $(f, g) (:= f+g\wt{c})$ satisfies $\theta(f, g)=0$. 
Then, taking mod $p$, we obtian $(f, g)$ goes to zero in 
$k[[x, y, z]] \oplus k[[x, y, z]] c$. 
This implies that $(f, g) = (pf', pg')$ for some $f', g' \in W(k)[\wt{x}, \wt{y}, \wt{z}]$. 
Since $p\theta(f', g')=0$ and $\wt{C}$ is $p$-torsion free, 
we get $\theta(f', g')=0$, which implies $(f', g')=(pf'', pg'')$. 
Then $f, g \in p^2 W(k)[\wt{x}, \wt{y}, \wt{z}]$. 
Repeating this procedure, we obtain 
\[
f, g \in \bigcap_{n \geq 1} p^n W(k)[[\wt{x}, \wt{y}, \wt{z}]] =0. 
\]
This completes the proof of Claim. 
\end{proof}

In what follows, the argument as in 
[Tanaka, 
Elliptic sigularities and threefold flops in positive characteristic, 6.13] works. 
\end{proof}

\begin{rem}
The above construction shows that $\wt{Y}^+$ is smooth over $W(k)$, because $\wt{Y}$ and $\wt{Y}^+$ are formally isomorphic. 
Moreover, $\wt{Y}^+ \to Z$ has at most one-dim fibres. 
\end{rem}


We have shown that the mixed-char flopping contraction 
$\wt{Y} \to \wt{Z}$ has a flop $\wt{Y}^+ \to \wt{Z}$. 
It is clear that this flop compatible with the char-zero flop, 
i.e., after taking the base change to the generic fibre over $W(k)$, this becomes the flop in char 0 
(taking char 0 means that take the open subset of $\Spec W(k)$ (the generic point) and its inverse images). 

Let us compare 
\begin{itemize}
    \item the char-p flop $Y^+$
    \item the sm 3-fold $\wt{Y}^+_p$ obtained by taking the mod p reduction of the mixed-char flop $\wt{Y}^+$. 
\end{itemize}
Since $\wt{Y}^+_p \to \wt{Z}_p = Z$ has at most one-dim fibres, 
this is a small birat contraction. 
Moreover, the anti-ample divisor on $Y$ becomes ample (over $Z$) 
on $\wt{Y}^+_p$. 
Thus these coincide, and hence $\wt{Y}^+_p\simeq Y^+$. 

\subsection{The case $g=11$}



Let $X$ be a smooth Fano threefold such that $\rho(X) = r_X =1$, 
$|-K_X|$ is very ample, and $(-K_X)^3 = 20$. 
By $(-K_X)^3 = 2g-2$, the last condition is equivalent to  $g=11$. 
It follows from \cite[Theorem 6.7]{FanoII} that $X$ contains a conic $\Gamma$. 
Let $\sigma : Y \to X$ be the blowup along $\Gamma$. 
Then $|-K_Y|$ is base point free and $-K_Y$ is big 
\cite[Proposition 7.2.]{FanoII}. 
Let $\psi : Y \to Z$ be the contraction that is obtained by taking the Stein factorisation of $\varphi_{|-K_Y|}$. 
Then $\psi$ is a birational contraction. 
By \cite[Proposition 7.3]{FanoII}, we get $\dim \Ex(\psi) \neq 2$. 
Hence either $-K_Y$ is ample or $\dim \Ex(\psi)=1$ (i.e., $\psi$ is a flopping contraction). 
Let $\psi^+ : Y^+ \to Z$ be the flop of $\psi : Y \to Z$. 
Take the contraction $\tau : Y^+ \to W$ of the $K_{Y^+}$-negative extremal ray. 
By \cite[Theorem 7.4]{FanoII}, it holds that 
$W = \P^3$ and $\tau$ is a blowup along a smooth rational curve $B$ of degree $6$. 
\[
\begin{tikzcd}
Y \arrow[d, "\sigma"'] \arrow[rd, "\psi"]& & Y^+ \arrow[ld, "\psi^+"'] \arrow[d, "\tau"]\\
X & Z & W=\P^3
\end{tikzcd}
\]
We shall construct lifts of this  diagram in reverse order. 
\begin{enumerate}
\item Lifts  of $Y^+$ and $W$. 
\item A lift of $Z$.
\item A lift of $Y$.
\item A lift of $X$. 
\end{enumerate}


\commentbox{For (2) and (4), it is enough to check that $R^1f_*\MO=0$ (in char p), 
which is much easier than below. Lifts preserve $\rho(-)$: $\rho(X) = \rho(X_0)$, 
so the nef thresholds must coincide. [Bernasconi-Brivio-Kawakami-Witaszek, Lifting globally F-split surfaces to characteristic zero], Theorem 2.14, proof of Prop 5.2}

(1) We have a $W(k)$-lift $\wt{W} =\P^3_{W(k)}$ of $W$.  
By Totaro's idea, the blowup centre $B$ lits to $\wt{W}$, which is denoted by 
$\wt{B}$. 
Let $\wt{Y}^+ \to \wt{W}$ be the blowup along $\wt{B}$. 

(2) Since $-K_{Y^+}$ is nef and big, so is $-K_{Y^+_0}$, 
where the subscript $(-)_0$ denotes the geometric generic fibre of $(-) \to \Spec W(k)$. 
Since $\Ex(\psi^+)$ is one-dimensional, $\Ex(\psi^+_0)$ is one-dimensional or empty. 
The latter case does not occur, as otherwise $Y^+_0$ would be a smooth Fano threefold obtained by taking a blowup of $\P^3$ along a smooth rational curve $B_0$ of degree $6$, which contradicts the classification table 
(cf.\ \cite[Table in Subsection 7.2]{FanoIV}, note that such a Fano threefold would satisfy $(-K)^3 =12$ if it existed). 

 Then $-K_{\wt{Y}}$ is semi-ample and big. 
Moreover, 
\[
0 \to \MO_{\wt Y^+}(-Y^+) \to \MO_{\wt Y^+} \to \MO_{Y^+} \to 0
\]
induces 
\[
H^0(\wt Y^+, -mK_{\wt Y^+}) \to H^0(Y^+, -mK_{Y^+}) \to 
H^1(\wt Y^+, -mK_{\wt Y^+} - Y^+) \simeq H^1(\wt Y^+, -mK_{\wt Y^+}) =0
\]
for $m \gg 0$. 
Here  the last vanishing holds by upper-semicontinuity and 
\[
H^i(Y^+, -mK_{Y^+}) \simeq H^i(Z, -mK_Z) =0
\]
for $i>0$. 
Therefore,  the induced morphism $\wt{\psi}^+ : \wt{Y}^+ \to \wt{Z}$ is a lift of 
$\psi^+.$ 


(3) This part has already settled in the previous subsection. 

% Pick an effective divisor $E_{Y^+}$ on $Y^+$ which is $\psi^+$-anti-ample. 
% Pick large integers $m, n \gg 0$, we set  
% \[
% L^+ := m( -nK_{Y^+} +E_{Y^+}), 
% \]
% which is a Cartier divisor. 
% Since $F_Y$ is $\psi$-ample, we see that $-nK_Y+ F_Y$ is ample, 
% which implies $Y = \Proj\,R(Y^+, L^+)$.

% Strategy: to prove $h^0(Y^+, dL^+)_p = h^0(Y^+, dL^+)_0$ (i.e., invariances of dimensions). 
% Then we may apply the Grauert theorem, so that 
% \[
% H^0(\wt{Y}^+, d\wt{L}^+) \otimes W/pW \simeq  H^0(Y^+, dL^+). 
% \]
% Then the flop should lift. 

%  In char p, we have the flop $Y$ of $Y^+$. 
%  Then 
%  \[
%  h^0(Y^+, dL^+) = h^0(Y, dL) = \chi(Y, dL) = \chi(Y, dm(-nK_Y +E)). 
%  \]
%  R-R. 





% We can take lifts $\wt D^+$. 
% Assume that 
% \begin{enumerate}
% \item[($\star$)] $R(\wt Y^+, \wt D^+)$ is finitelt gerated and 
% \[
% R(\wt Y^+, \wt D^+) \otimes_{W(k)} W(k)/pW(k) \simeq R(Y^+, D^+). 
% \]
% \end{enumerate}
% Then $\Proj R(\wt Y^+, \wt D^+)$ is a flop of $\wt Y^+ \to \wt Z$, 
% and it is a lift of $Y$. 

% Hence it is enough to show ($\star$). 
% Fix an integer $d \geq 0$. 
% It is probably enough to prove the surjectivity of  
% \[
% H^0(\wt Y^+, dm( -K_{Y^+} +\epsilon F_{Y^+})) \to 
% H^0(Y^+,  dm(-K_{Y^+} +\epsilon F_{Y^+}))
% \]
% and the vanishing of higher cohomologies. 



(4) 
Since $-K_Y$ is nef and big, also $-K_{Y_0}$ is nef and big. 
As $\rho(Y_0)=2$ and $-K_{Y_0}$ is trivial for $\psi_0$, 
we have a unique $K_{Y_0}$-negative extremral ray. 
Recall that $K_Y = \sigma^*K_X + E$. 
Hence $-K_Y+E = -\sigma^*K_X$ is nef and big but not ample. 
Consider the nef threshold $-K_{Y_0} + \lambda E_0$ in char 0. 
Note that $-K_{Y_0} + E_0$ is nef and big, whilst $-K_{Y_0} +E_0$ might be ample. 

We have 
\[
H^0(\wt{Y}, m(-K+E)) \to H^0(Y, m(-K+E)) \to H^1(\wt{Y}, m(-K+E) -Y) =H^1(\wt{Y}, m(-K+E))= 0
\]
for $m \gg 0$ by the upper semi. 
Then we get 
\[
\wt{Y} \to \wt{X}
\]
which is a lift of $Y \to X$. 
Then $X_0$ is a smooth Fano threefold with $\rho(X_0)=1$ and 
$(-K_{X_0})^3 = (-K_X)^3 = 20$. 
This is absurd. 


% \vspace{20mm}



% Let us show that $-K_{Y_0}+E_0$ is not ample. 
% We have that 
% \[
% \wt{\sigma} : \wt{Y} \to \wt{X}
% \]
% be the contraction by the semi-ample and big $-K_{\wt Y} +\wt{E}$. 
% Then char 0 fibres does not change. In particular, $\wt{\sigma}$ is a small birational contraction, and hence $\wt{X}$ is not $\Q$-factorial. 
% On the other hand, $\wt{X} \to \Spec W(k)$ is a smooth flat morphism. Hence $\wt{X}$ is regular, which is absurd. 
% (Or, consider the deformation invariant value $(-K)^3$) 


% Then $-K_{Y_0} + E_0$ is not ample. 
% We get a contraction
% \[
% \wt{\sigma} : \wt{Y} \to \wt{X}. 
% \]
% Then $(-K_{X_0})^3 = (-K_X)^3 = 20$, which is a contradiction. 




 

% Since fibre dimension is one in char $p$, this holds also in char 0. 
% Hence the char 0 contraction is also of type $E_1$. 
% $\deg \Gamma$ and $g(\Gamma)$ can be computed by  deformation invariant values: 
% $(-K_Y)^3$ and $(-K_Y)^2 \cdot E$, and hence $Y_0 \to X_0$ is a blowup along a smooth conic. 
% Hence $(-K_{X_0})^3$




% Suppose that $-K_{Y_0}+E_0$ is ample. Then $-K_{Y_0} + \lambda E_0$ is nef and big. 
% Hence its contraction $\varphi : Y_0 \to V$ is birational. 
% Then $K_{Y_0} = \varphi^*K_V + \lambda E_0$ with $\lambda >0$. 
% By the classification of extremal rays [Mori], 
% $\varphi$ is of type $E_2$ and $\lambda =2$. 
% Therefore, $V$ is a smooth Fano threefold with $\rho(V) =1$
% \[
% (-K_V)^3 -8 = (-K_{Y_0})^3 = (-K_Y)^3 = (-K_X)^3 -6 =22 -2 - 6 = 14. 
% \]
% Hence $(-K_V)^3 = 22$. 
% By classification, $\rho(V) = r_V=1$,  $-K_V$ is very ample, and $g_V=12$. 
% Unfortunately, no contradiction with the classification table...



% % \begin{remark}
% % In order to overcome the above (4), how about considering the contraction: 
% % \[
% % \wt{Y} \to \wt{X}, 
% % \]
% % induced by $-K_{\wt{Y}} +\wt{E}$. 
% % Then this is a birational morphism of 4-folds over $W(k)$ s.t. 
% % the char 0 fibres are the same, but char p fibres differs. 
% % \[
% % \wt{X} 
% % \]
% % \end{remark}



% \begin{lem}
% Let $W :=\P^3$ and take a smooth rational curve $B$ of deg $6$. 
% Let $\tau : V \to W$ be the blwoup along $B$. 
% Set $D := \Ex(\tau)$. 
% Assume that $-K_V$ is nef and big but not ample. 
% Assume that the contraction $V \to Z$  by $-K_V$ is a flopping contraction. 
% Let $V^-$ be the flop.  
% Let $\rho : V^- \to U$ be the contraction of $K$-neg ext ray. 
% \end{lem}
% We have 
% \begin{itemize}
% \item $(-K_V)^3 = 2g-16 =6$
% \item $(-K_V)^2D = \deg +2g(\Gamma)-2  =4$. 
% \item $(-K_V) \cdot D^2 =-2$
% \end{itemize}
% $H := \tau^* \MO(1)$. 
% We can write $F \sim -\alpha K_{V^-} -\beta D^-$. 
% \[
% F \cdot (-K_V)^2 = (-K)^2(-\alpha K_{V^-} -\beta D^-) = (-K)^3 \alpha -(-K)^2D \beta = 6\alpha -4\beta. 
% \]
% \[
%  F^2 (-K_{V^-}) = (-K)^3\alpha^2- (-K)^2D 2\alpha \beta  + (-K)D^2 \beta^2
% =6\alpha^2  -8\alpha \beta -2\beta^2. 
% \]



% Type $D$: this is impossible, because the solutions of $6x^2 -8x -2=0$ are irrational. 

% Type $C$: $F^2 (-K)=2$. 
% Then 
% \[
% 3\alpha^2 -4\alpha\beta -\beta^2 = 1. 
% \]


\subsection{$g=12, 8, 7, 6$}

If $g=12$, then the same argument as in $g=11$ works by 
starting with a point blowup.  So lifts to $W(k)$. 
%using the point-

Assume $g=8$. 
Use a point blowup. 
Div cont does not occur. 
We need to check the details. 


For the case when $g=7$, the sitation is the same as $g=8$ by using the conic blowup. 


$g=6$: follow from Debbare-Kuznetsov. We get CI inside a Grassmannian-like variety. So litable. 


\subsection{Del Pezzo fibrations}

\begin{prop}
    Let $f\colon X\to B$ be a del Pezzo fibration.
    Suppose that the following holds.
    \begin{enumerate}
        \item A general fibre $D$ is smooth and satisfies Bott vanishing.
        \item For a non-reduced fibre $nF$, we have $F$ is normal and log liftable.
    \end{enumerate}
    Then $X$ lifts to $H^1(X, \Omega^1_X(K_X))=0$.
    In particular, $X$ lifts to $W(k)$.
\end{prop}
\begin{proof}
    By the conormal exact sequence, we have
    \[
    0\to \sO_D(K_D) \to \Omega^1_X(K_X)|_D \to \Omega^1_D(K_D) \to 0.
    \]
    Together with Bott vanishing on $D$, we have $H^1(D, \Omega^1_X(K_X)|_D)=0$.

    We have an exact sequence
    \[
    0\to \Omega^1_X(K_X-mD) \to \Omega^1_X(K_X-(m-1)D) \to \Omega^1_X(K_X)|_D \to 0
    \]
    for all $m\geq 1$. Note that $D|_D=0$.
    Thus, it suffices to show that
    \[
    H^1(X,\Omega^1_X(K_X-mD))=0
    \]
    for some $m\gg0$.
    By duality, it suffices to show that
    \[
    H^2(X, \Omega^2_X(mD-K_X))=0.
    \]

    Consider the spectral sequence
    \[
    H^p(B, R^qf_{*}\Omega^2_X(mD-K_X)) \Rightarrow H^{p+q}(X,\Omega^2_X(mD-K_X)).
    \]
    By Serre vanishing, we have \[H^p(B, R^qf_{*}\Omega^2_X(mD-K_X))=H^p(B, R^qf_{*}\Omega^2_X(-K_X)\otimes \sO_B(mb))=0\] for $p>0$ and  $m\gg0$, where $b\in B$ is a closed point.

    Then, we have
    \[
    H^2(X, \Omega^2_X(mD-K_X))=H^0(B, R^2f_{*}\Omega^2_X(-K_X)\otimes \sO_B(mb)).
    \]
    Thus, it suffices to show that
    \[
    R^2f_{*}\Omega^2_X(-K_X)=0.
    \]
    By the formal function theorem, the assertion can be reduced to the following claim:
    \begin{claim}
        We have $H^2(nF,\Omega^2_X(-K_X)|_{nF})=0$ for all $n>0$.
    \end{claim}
    \begin{proof}
        We note $F|_F=0$.
        By snake lemma, we obtain an exact sequence
        \[
        0\to \Omega^2_X(-K_X)|_F \to \Omega^2_X(-K_X)|_{nF} \to \Omega^2_X(-K_X)|_{(n-1)F} \to 0.
        \]
        Thus, it suffices to show that 
        \[
        H^2(F,\Omega^2_X(-K_X)|_{F})=0.
        \]
        Since $F$ is normal, we have an exact sequence
        \[
        0\to \Omega^{[1]}_F(-K_F)\to \Omega^2_X(-K_X)|_F \to \sO_{F}.
        \]
        Let $\mathcal{B}\subset \sO_F$ be the image of the last map.
        Since $\Supp(\sO_F/\mathcal{B})$ has codimension at least two, we have
        \[
        H^2(F,\mathcal{B})=H^2(F, \sO_F)=0.
        \]
        We also have
        \[
        H^2(F, \Omega^{[1]}_F(-K_F))\cong H^0(F, \Omega^{[1]}_F(K_F))=0
        \]
        since $F$ is log liftable.
        Thus, we conclude $H^2(F,\Omega^2_X(-K_X)|_{F})=0$.
    \end{proof}
    
\end{proof}
